Modeling Gestalt Visual Reasoning on the Raven's Progressive Matrices Intelligence Test Using Generative Image Inpainting Techniques

Psychologists recognize Raven's Progressive Matrices as a very effective test of general human intelligence. While many computational models have been developed by the AI community to investigate different forms of top-down, deliberative reasoning on the test, there has been less research on bottom-up perceptual processes, like Gestalt image completion, that are also critical in human test performance. In this work, we investigate how Gestalt visual reasoning on the Raven's test can be modeled using generative image inpainting techniques from computer vision. We demonstrate that a self-supervised inpainting model trained only on photorealistic images of objects achieves a score of 27/36 on the Colored Progressive Matrices, which corresponds to average performance for nine-year-old children. We also show that models trained on other datasets (faces, places, and textures) do not perform as well. Our results illustrate how learning visual regularities in real-world images can translate into successful reasoning about artificial test stimuli. On the flip side, our results also highlight the limitations of such transfer, which may explain why intelligence tests like the Raven's are often sensitive to people's individual sociocultural backgrounds.

==> AAAI 2020 - Ravens Paper (1)/table_cpmnorms.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!} {

\begin{tabular}{c|llllllllllllllll}

\hline
\multirow{2}{*}{Percentile points} & \multicolumn{16}{c}{Age}                                                      \\
                                   & 11 & 10$\nicefrac{1}{2}$ & 10 & 9$\nicefrac{1}{2}$  & 9  & 8$\nicefrac{1}{2}$  & 8  & 7$\nicefrac{1}{2}$  & 7  & 6$\nicefrac{1}{2}$  & 6  & 5$\nicefrac{1}{2}$  & 5  & 4$\nicefrac{1}{2}$  & 4  & 3$\nicefrac{1}{2}$  \\ \hline
95                                 & 35 & 34 & 33 & 33 & 32 & 31 & 30 & 29 & 28 & 27 & 26 & 25 & 24 & 22 & 21 & 20 \\
90                                 & 34 & 33 & 32 & 31 & 30 & 29 & 28 & 28 & 27 & 26 & 24 & 23 & 22 & 20 & 19 & 17 \\
75                                 & 32 & 31 & 30 & 29 & 28 & 27 & 26 & 25 & 23 & 22 & 20 & 19 & 18 & 16 & 15 & 14 \\
50                                 & 29 & 28 & 27 & 26 & 25 & 23 & 22 & 21 & 19 & 18 & 16 & 15 & 14 & 12 & 11 & 10 \\
25                                 & 26 & 25 & 23 & 22 & 21 & 19 & 18 & 17 & 15 & 14 & 12 & 11 & 10 & 8  & 7  & -  \\
10                                 & 22 & 21 & 19 & 18 & 17 & 15 & 14 & 13 & 12 & 10 & 9  & 7  & -  & -  & -  & -  \\
5                                  & 20 & 19 & 17 & 16 & 15 & 13 & 12 & 11 & 9  & 8  & -  & -  & -  & -  & -  & -  \\ \hline
\end{tabular}

}
\caption[]{Amended norms for Colored Progressive Matrices \\ Ages $5 \nicefrac{1}{2}$ - 11, Extrapolated $3 \nicefrac{1}{2}$ - 5}
\end{table*}

==> AAAI 2020 - Ravens Paper (1)/table_ravenmodels.tex <==
\begin{tabularx}{\textwidth}
{@{} l X X X X @{}}
\toprule
    % \multicolumn{2}{c}{Part} \\
    % \cmidrule(r){1-2}
    Reference
    & Inputs
    & Type
    & Approach
    & Evaluation\\
\midrule
    \cite{carpenter1990one}
        & 
        &
        &
        &\\
        
    \cite{kunda2013computational}
        & 
        &
        &
        &\\
        
    \cite{strannegaard2013anthropomorphic}
        & 
        &
        &
        &\\
        
    \cite{lovett2017modeling}
        & 
        &
        &
        &\\
        
    3D Objects on Turntable 
        & 
        &
        &
        &\\
        
    3D Object
        & 
        &
        &
        &\\
        
    Intel Egocentric$^{4,5}$
        & 
        &
        &
        &\\
        
    EPFL-GIMS08
        & 
        &
        &
        &\\
        
    RGB-D$^{2}$
        & 
        &
        &
        &\\
        
    BigBIRD$^{2}$ 
        & 
        &
        &
        &\\
\bottomrule
%\multicolumn{5}{@{} l}
%{\textit{
%notes
%}} \\
\end{tabularx}

==> AAAI 2020 - Ravens Paper (1)/table_results.tex <==
\begin{table}
    % \centering
    
    % \resizebox{\linewidth}{!}{
    % \resizebox{0.5\textwidth}{!}{\begin{minipage}{\textwidth}
    \begin{adjustbox}{angle=90, max height=20cm}
    \begin{tabular}{c|cccccccccccc|cccccccccccc|cccccccccccc|c|c|c|c} 
    \hline
    \multirow{2}{*}{}         & \multicolumn{12}{c|}{A}                                                                                                                                          & \multicolumn{12}{c|}{AB}                                                                                                                                     & \multicolumn{12}{c|}{B}                                                                                                                           & \multirow{2}{*}{C} & \multirow{2}{*}{D} & \multirow{2}{*}{E}    & \multirow{2}{*}{CPM}  \\
                              & 1          & 2           & 3          & 4          & 5          & 6           & 7           & 8           & 9           & 10          & 11         & 12          & 13          & 14          & 15          & 16          & 17          & 18          & 19          & 20          & 21          & 22          & 23          & 24          & 25          & 26          & 27          & 28          & 29          & 30     & 31          & 32         & 33     & 34         & 35           & 36          &                    &                    &                       &                       \\ 
    \hline
    \multirow{2}{*}{Imagenet} & $\bullet $ & $\bullet $  & $\bullet $ & $\bullet $ & $\bullet $ & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &            &             & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &             & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &             & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &        & $\bullet $  &            &        &            &              & $\bullet $    &                    &                    &                       &                       \\
                              & \multicolumn{12}{c|}{10}                                                                                                                                         & \multicolumn{12}{c|}{10}                                                                                                                                     & \multicolumn{12}{c|}{7}                                                                                                                           & 1                  & 1                  & 6                     & 27                    \\ 
    \cline{2-37}
    \multirow{2}{*}{CelebA}   &            &             &            &            &            & $\bullet $  &             &             & $\bullet $  & $\bullet $  &            &             & $\bullet $  &             &             & $\bullet $  &             &             & $\bullet $  &             & $\bullet $  &             &             &             & $\bullet $  & $\bullet $  &             &             & $\bullet $  &        &             & $\bullet $ &        &            &              &               &                    &                    &                       &                       \\
                              & \multicolumn{12}{c|}{3}                                                                                                                                          & \multicolumn{12}{c|}{4}                                                                                                                                      & \multicolumn{12}{c|}{4}                                                                                                                           & 1                  & 0                  & 3                     & 11                    \\ 
    \cline{2-37}
    \multirow{2}{*}{DTD}      & $\bullet $ & $\bullet $  & $\bullet $ & $\bullet $ & $\bullet $ & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &            & $\bullet $  & $\bullet $  &             & $\bullet $  & $\bullet $  &             & $\bullet $  &             &             &             &             &             &             &             &  $\bullet $ &             &             & $\bullet $  &         &            &            &        &            &              & $\bullet $    &                       &                    &                       &   \\
                              & \multicolumn{12}{c|}{11}                                                                                                                                         & \multicolumn{12}{c|}{4}                                                                                                                                      & \multicolumn{12}{c|}{3}                                                                                                                           & 1                  & 1                  & 5                     & 18                    \\ 
    \cline{2-37}
    \multirow{2}{*}{Places2}  &            &             &            & $\bullet $ &            & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &            & $\bullet $  & $\bullet $  &             &             & $\bullet $  &             & $\bullet $  &             &             &             & $\bullet $  &             &             & $\bullet $  & $\bullet $  & $\bullet $  &             & $\bullet $  &        &             &            &        &            & $\bullet $  & $\bullet $  &                    &                    &                       &                       \\
                              & \multicolumn{12}{c|}{7}                                                                                                                                          & \multicolumn{12}{c|}{4}                                                                                                                                      & \multicolumn{12}{c|}{6}                                                                                                                           & 1                  & 0                  & 3                     & 17                    \\
    \hline
    
    \end{tabular}
    \end{adjustbox}
    % \end{minimap}}
    \caption{some caption}
    \label{tab:another_label}
\end{table}

==> table_cpmnorms.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!} {

\begin{tabular}{c|llllllllllllllll}

\hline
\multirow{2}{*}{Percentile points} & \multicolumn{16}{c}{Age}                                                      \\
                                   & 11 & 10$\nicefrac{1}{2}$ & 10 & 9$\nicefrac{1}{2}$  & 9  & 8$\nicefrac{1}{2}$  & 8  & 7$\nicefrac{1}{2}$  & 7  & 6$\nicefrac{1}{2}$  & 6  & 5$\nicefrac{1}{2}$  & 5  & 4$\nicefrac{1}{2}$  & 4  & 3$\nicefrac{1}{2}$  \\ \hline
95                                 & 35 & 34 & 33 & 33 & 32 & 31 & 30 & 29 & 28 & 27 & 26 & 25 & 24 & 22 & 21 & 20 \\
90                                 & 34 & 33 & 32 & 31 & 30 & 29 & 28 & 28 & 27 & 26 & 24 & 23 & 22 & 20 & 19 & 17 \\
75                                 & 32 & 31 & 30 & 29 & 28 & 27 & 26 & 25 & 23 & 22 & 20 & 19 & 18 & 16 & 15 & 14 \\
50                                 & 29 & 28 & 27 & 26 & 25 & 23 & 22 & 21 & 19 & 18 & 16 & 15 & 14 & 12 & 11 & 10 \\
25                                 & 26 & 25 & 23 & 22 & 21 & 19 & 18 & 17 & 15 & 14 & 12 & 11 & 10 & 8  & 7  & -  \\
10                                 & 22 & 21 & 19 & 18 & 17 & 15 & 14 & 13 & 12 & 10 & 9  & 7  & -  & -  & -  & -  \\
5                                  & 20 & 19 & 17 & 16 & 15 & 13 & 12 & 11 & 9  & 8  & -  & -  & -  & -  & -  & -  \\ \hline
\end{tabular}

}
\caption[]{Amended norms for Colored Progressive Matrices \\ Ages $5 \nicefrac{1}{2}$ - 11, Extrapolated $3 \nicefrac{1}{2}$ - 5}
\end{table*}

==> table_ravenmodels.tex <==
\begin{tabularx}{\textwidth}
{@{} l X X X X @{}}
\toprule
    % \multicolumn{2}{c}{Part} \\
    % \cmidrule(r){1-2}
    Reference
    & Inputs
    & Type
    & Approach
    & Evaluation\\
\midrule
    \cite{carpenter1990one}
        & 
        &
        &
        &\\
        
    \cite{kunda2013computational}
        & 
        &
        &
        &\\
        
    \cite{strannegaard2013anthropomorphic}
        & 
        &
        &
        &\\
        
    \cite{lovett2017modeling}
        & 
        &
        &
        &\\
        
    3D Objects on Turntable 
        & 
        &
        &
        &\\
        
    3D Object
        & 
        &
        &
        &\\
        
    Intel Egocentric$^{4,5}$
        & 
        &
        &
        &\\
        
    EPFL-GIMS08
        & 
        &
        &
        &\\
        
    RGB-D$^{2}$
        & 
        &
        &
        &\\
        
    BigBIRD$^{2}$ 
        & 
        &
        &
        &\\
\bottomrule
%\multicolumn{5}{@{} l}
%{\textit{
%notes
%}} \\
\end{tabularx}

==> table_results.tex <==
\begin{table}
    % \centering
    
    % \resizebox{\linewidth}{!}{
    % \resizebox{0.5\textwidth}{!}{\begin{minipage}{\textwidth}
    \begin{adjustbox}{angle=90, max height=20cm}
    \begin{tabular}{c|cccccccccccc|cccccccccccc|cccccccccccc|c|c|c|c} 
    \hline
    \multirow{2}{*}{}         & \multicolumn{12}{c|}{A}                                                                                                                                          & \multicolumn{12}{c|}{AB}                                                                                                                                     & \multicolumn{12}{c|}{B}                                                                                                                           & \multirow{2}{*}{C} & \multirow{2}{*}{D} & \multirow{2}{*}{E}    & \multirow{2}{*}{CPM}  \\
                              & 1          & 2           & 3          & 4          & 5          & 6           & 7           & 8           & 9           & 10          & 11         & 12          & 13          & 14          & 15          & 16          & 17          & 18          & 19          & 20          & 21          & 22          & 23          & 24          & 25          & 26          & 27          & 28          & 29          & 30     & 31          & 32         & 33     & 34         & 35           & 36          &                    &                    &                       &                       \\ 
    \hline
    \multirow{2}{*}{Imagenet} & $\bullet $ & $\bullet $  & $\bullet $ & $\bullet $ & $\bullet $ & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &            &             & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &             & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &             & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &        & $\bullet $  &            &        &            &              & $\bullet $    &                    &                    &                       &                       \\
                              & \multicolumn{12}{c|}{10}                                                                                                                                         & \multicolumn{12}{c|}{10}                                                                                                                                     & \multicolumn{12}{c|}{7}                                                                                                                           & 1                  & 1                  & 6                     & 27                    \\ 
    \cline{2-37}
    \multirow{2}{*}{CelebA}   &            &             &            &            &            & $\bullet $  &             &             & $\bullet $  & $\bullet $  &            &             & $\bullet $  &             &             & $\bullet $  &             &             & $\bullet $  &             & $\bullet $  &             &             &             & $\bullet $  & $\bullet $  &             &             & $\bullet $  &        &             & $\bullet $ &        &            &              &               &                    &                    &                       &                       \\
                              & \multicolumn{12}{c|}{3}                                                                                                                                          & \multicolumn{12}{c|}{4}                                                                                                                                      & \multicolumn{12}{c|}{4}                                                                                                                           & 1                  & 0                  & 3                     & 11                    \\ 
    \cline{2-37}
    \multirow{2}{*}{DTD}      & $\bullet $ & $\bullet $  & $\bullet $ & $\bullet $ & $\bullet $ & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &            & $\bullet $  & $\bullet $  &             & $\bullet $  & $\bullet $  &             & $\bullet $  &             &             &             &             &             &             &             &  $\bullet $ &             &             & $\bullet $  &         &            &            &        &            &              & $\bullet $    &                       &                    &                       &   \\
                              & \multicolumn{12}{c|}{11}                                                                                                                                         & \multicolumn{12}{c|}{4}                                                                                                                                      & \multicolumn{12}{c|}{3}                                                                                                                           & 1                  & 1                  & 5                     & 18                    \\ 
    \cline{2-37}
    \multirow{2}{*}{Places2}  &            &             &            & $\bullet $ &            & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  & $\bullet $  &            & $\bullet $  & $\bullet $  &             &             & $\bullet $  &             & $\bullet $  &             &             &             & $\bullet $  &             &             & $\bullet $  & $\bullet $  & $\bullet $  &             & $\bullet $  &        &             &            &        &            & $\bullet $  & $\bullet $  &                    &                    &                       &                       \\
                              & \multicolumn{12}{c|}{7}                                                                                                                                          & \multicolumn{12}{c|}{4}                                                                                                                                      & \multicolumn{12}{c|}{6}                                                                                                                           & 1                  & 0                  & 3                     & 17                    \\
    \hline
    
    \end{tabular}
    \end{adjustbox}
    % \end{minimap}}
    \caption{some caption}
    \label{tab:another_label}
\end{table}
